X-Risk Analysis for AI Research

Artificial intelligence (AI) has the potential to greatly improve society, but as with any powerful technology, it comes with heightened risks and responsibilities. Current AI research lacks a systematic discussion of how to manage long-tail risks from AI systems, including speculative long-term risks. Keeping in mind the potential benefits of AI, there is some concern that building ever more intelligent and powerful AI systems could eventually result in systems that are more powerful than us; some say this is like playing with fire and speculate that this could create existential risks (x-risks). To add precision and ground these discussions, we provide a guide for how to analyze AI x-risk, which consists of three parts: First, we review how systems can be made safer today, drawing on time-tested concepts from hazard analysis and systems safety that have been designed to steer large processes in safer directions. Next, we discuss strategies for having long-term impacts on the safety of future systems. Finally, we discuss a crucial concept in making AI systems safer by improving the balance between safety and general capabilities. We hope this document and the presented concepts and tools serve as a useful guide for understanding how to analyze AI x-risk.

==> comments.tex <==
Scaling laws
- dual nature

Differential privacy

Causality
- main purpose is to enable learning from less data, so general causality papers lean towards capabilities

Fairness

Interpretability

Debate

Iterated amplification




For credit scoring:
- first-world concerns
- direct risk reduction, but not an x-risk
- for machine ethics, would the problem not being solved lead to significant loss of life?





==> old_content_dump.tex <==
From 4-long-term-impact.tex


Would outstanding capabilities plausibly straightforwardly render this work irrelevant?

If this problem were not entirely solved, would that make advanced systems dramatically less economically useful?

Is working on this earlier likely to have positive compounding effects (such as field-building effects)?

Would advanced systems be thought highly unintelligent if they could not have the property that you are aiming for?

Is this problem a continuous problem or something that can be entirely solved (e.g., an off-switch)?

Is it beneficial to have models that are superhuman at this task? Are there different levels of superhuman capabilities, or is there a ceiling around human-level?
Would achieving human-level performance at this task not be sufficiently safe?

relevance to advanced models or are these actually just low-level cognitive skills that do not affect inherent hazards? (but perception is useful for monitoring)

External validity or ecological validity of the environments or experiments; does this work in many settings?
Is this consistently useful across different scales? Does this improve the scaling law?

Does this method introduce or is it contingent on handcrafted knowledge, features, or designs? (Bitter Lesson)

Does this require humans to be in the loop or rely on human reliability?

Does the utility of this idea depend on specifics of models, e.g., the presence of channels?

Is this work highly dependent on a particular method?

Is this work useful for state-of-the-art systems?
Is this work useful for age-tested systems as well?
Is this only making old-school algorithms and not state-of-the-art systems safer?

Is the performance substantially better previous methods, or is the performance improvement minor?

Does it provide a Pareto improvement or is it nearly Pareto optimal?

Does this require substantially more compute, pretraining data, or human annotation?

Is the method easy to incorporate with existing systems?

Does the work require training tricks or extensive hyperparameter tuning?

Is the result ``nice to know'' but has time-bound or method-bound implications? Does this knowledge impel future action?

Is this a speculative, untested proposal?

Is this only demonstrated on toy problems or assuming toy models?

Are there clear ways in which this could prevent the sudden loss of life at a large-scale? (risk analysis?)

Does this increase safety by strongly trading off against raw intelligence?




















From 5-externalities.tex


Is the way you are improving safety by simultaneously advancing other capabilities?
Does this advance the study of safety as a consequence of advancing the study of AI more generally?


Here we take ``general tasks'' to mean the set of tasks humans might reasonably want models perform well on. Obviously there's the no free lunch theorem, so we're considering a set of natural tasks that might lie on a low-dimensional manifold.

Is it inert? If not, does it marginally improve safety more than capabilities?

Does this improve performance on general tasks? If this targets subtasks, what properties of these subtasks make it especially useful for safety?

Does this primarily improve the general accuracy, scalability, or efficiency of models?

How is this separate from improving general classification, prediction, generation, data compression, instruction execution, reasoning, planning, optimization, or sequential decision making capabilities?

How is this separate from typical economically incentivized arbitrary goals (a large share of the default incentives governing AI development)? How is this relatively underincentivized?

Do people who care nothing for reliability or alignment have this as a top priority?
Would multiple different groups who care nothing for reliability or alignment find this work useful?


Is the objective you are trying to increase weakly correlated or negatively correlated with upstream performance?

Does this hardly advance upstream performance?

Does this method have important analogues in security or high-risk technologies (e.g., anomaly detection for information assurance, robustness for reducing component failures in extreme conditions, etc.)?

In humans is this goal something that is not strictly a function of cognitive ability (e.g., moral tendencies)?
In humans, is this ability highly predicted by general cognitive ability?

Does this incentivize giving AI systems elevated computer system privileges or capabilities (e.g., HTTP Post requests)? (their action space, communication channels, and access to information should be minimal.)

Does this paper simultaneously introduce several new capabilities?

Does this paper work towards recursive self-improvement or help automate AI research?

Does this incentivize work towards agents that do not have time-bound goals or clear, objective, known-before-hand final goal?

Bad question: would this be economically valuable? would be have incentives to do this? (people are incentivized to not go extinct; can't try to make it so that no one sees it as valuable; too tall of an order)




\newpage
\section{X-Risk Sheet}
\subsection{Risk Models}
\begin{enumerate}[leftmargin=*]
    \item How is this work intended to reduce existential risks from advanced AI systems?\quad 
    
    \item If this work directly reduces existential risks, what are the main failure mode(s) or hazards that it directly affects?\quad 

    \item If this work reduces existential risks in a diffuse manner, what are the main contributing factors that it affects?\quad 

    \item Are there clear ways in which this could prevent the sudden loss of life at a large-scale? If so, what is a scenario?\quad 
\end{enumerate}

\subsection{Capabilities Analysis}

\begin{enumerate}[resume,leftmargin=*]
    \item Does this primarily improve general prediction, classification, state estimation, efficiency, scalability, generation, data compression, executing clear instructions, reasoning, planning, researching, optimization, (self-)supervised learning, sequential decision making, or similar capabilities? \hfill $\boxtimes$

    \item Does this advance safety along with advancing capabilities or the study of AI? \hfill $\boxtimes$

    \item In humans, is this ability highly predicted by general cognitive ability? \hfill $\boxtimes$

    \item Does this paper work towards recursive self-improvement, open-ended goals, or models with elevated computer system access? \hfill $\boxtimes$

    \item Would numerous different groups with goals that do not include reliability or alignment find this work useful? \hfill $\boxtimes$

    \item How does this increase safety more than it increases capabilities?\quad 

    \item What is a way in which this hastens AI capabilities or the onset of x-risks?\quad 
\end{enumerate}

\subsection{Long-Term Impact}

\begin{enumerate}[resume,leftmargin=*]
    \item Do the findings decisively depend on model scale, hyperparameters, datasets/environments, strong theoretical assumptions, or a different machine learning paradigm? \hfill $\boxtimes$

    \item Is it infeasible to test ideas from this work now? \hfill $\boxtimes$

    \item Does this require handcrafted knowledge, expert humans, or human reliability? \hfill $\boxtimes$





    \item Would a human-level AI fulfill this safety property or goal? (That is, the property asymptotes around human-level and does not scale with intelligence beyond human-levels.) \hfill $\boxtimes$

    \item Does work towards this safety approach strongly trade off against raw intelligence, other capabilities, or economic usefulness? \hfill $\square$

    \item How does this work translate to the improved safety of far-future advanced AI systems?\quad 
    
    \item In what ways is this work likely to have positive compounding effects, such as field-building effects, or other forms of counterfactual impact on the safety of advanced AI?\quad
\end{enumerate}

\subsection{Other Considerations}
\begin{enumerate}[resume,leftmargin=*]
    \item What uncertainties do you have about this work and its relation to existential risk?\quad 

    \item What other comments about this work and existential risk are worth mentioning?\quad 
\end{enumerate}






\def\impacttext{In this section, please analyze how this work shapes the process that will lead to advanced AI and how it steers the process in a safer direction.}

\def\qone{\textbf{Overview.} How is this work intended to reduce existential risks from advanced AI systems?\quad }

\def\qtwo{\textbf{Direct Effects.} If this work directly reduces existential risks, what are the main hazards, vulnerabilities, failure mechanisms, or failure modes that it directly affects?\quad }

\def\qthree{\textbf{Diffuse Effects.} If this work reduces existential risks indirectly or diffusely, what are the main contributing factors that it affects?\quad }


\def\qfour{\textbf{Severity Threshold.} What is a future scenario in which this research direction could prevent the sudden, large-scale loss of life, if applicable?\quad }

\def\qfive{\textbf{Result Robustness.} Do the findings fail to hold across experimental design choices, such as different model sizes, hyperparameters, datasets, or environments? Are the ideas not tested on cutting-edge tasks? Or do they depend on strong theoretical assumptions, a different machine learning paradigm, and so on? \hfill }

\def\qsix{\textbf{Limited Testing.} Is it infeasible to test ideas from this work now, or are the ideas not tested on cutting-edge tasks? \hfill }

\def\qseven{\textbf{Problem Difficulty.} Would an AI with the abilities of an average human fulfill this safety property or goal? Or does the property not scale nor improve with intelligence beyond human-levels? \hfill }

\def\qeight{\textbf{Human Unreliability.} Does this approach require handcrafted knowledge, expert humans, or human reliability? \hfill }

\def\qnine{\textbf{Competitive Pressures.} Does work towards this safety approach strongly trade off against raw intelligence, other capabilities, or short-term economic usefulness? \hfill }

\def\qten{\textbf{Overview.} How does this increase safety more than it increases other capabilities?\quad }

\def\qeleven{\textbf{Red Teaming.} What is a way in which this hastens AI capabilities or the onset of x-risks?\quad }

\def\qtwelve{\textbf{Generality Indicator.} Are tasks that have been previously considered the subject of capabilities research advanced by this work? \hfill }

\def\qthirteen{\textbf{Hazardous Means.} Does this paper work towards or incentivize work on recursive self-improvement, open-ended goals, or models with elevated computer system access? \hfill }

\def\qfourteen{\textbf{General Ends.} Does this primarily improve or facilitate research on general prediction, classification, state estimation, efficiency, scalability, generation, data compression, executing clear instructions, reasoning, planning, researching, optimization, (self-)supervised learning, sequential decision making, or similar capabilities? \hfill }

\def\qfifteen{\textbf{Correlation With Intelligence.} Is the analyzed capability known to be highly predicted by raw intelligence, general cognitive ability, or educational attainment in humans? \hfill }

\def\qsixteen{\textbf{Safety via Capabilities.} Does this advance safety along with, or as a consequence of, advancing other capabilities or the study of AI? \hfill }

\def\qseventeen{What clarifications for previous questions are worth mentioning?\quad }

\def\qeighteen{What other comments or uncertainties about this work and existential risk are worth mentioning?\quad }


\def\externalitiestext{In this section, please analyze how the contribution relates to general capabilities and how it affects the balance between safety and hazards from general capabilities.}
















